PFL-GAN: When Client Heterogeneity Meets Generative Models in Personalized Federated Learning

Recent advances of generative learning models are accompanied by the growing interest in federated learning (FL) based on generative adversarial network (GAN) models. In the context of FL, GAN can capture the underlying client data structure, and regenerate samples resembling the original data distribution without compromising the private raw data. Although most existing GAN-based FL works focus on training a global model, Personalized FL (PFL) sometimes can be more effective in view of client data heterogeneity in terms of distinct data sample distributions, feature spaces, and labels. To cope with client heterogeneity in GAN-based FL, we propose a novel GAN sharing and aggregation strategy for PFL. The proposed PFL-GAN addresses the client heterogeneity in different scenarios. More specially, we first learn the similarity among clients and then develop an weighted collaborative data aggregation. The empirical results through the rigorous experimentation on several well-known datasets demonstrate the effectiveness of PFL-GAN.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.  


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
		Sigch-a sample bibliography renamed
		Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
		Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
		Corrected the bug with acmPrice.
		Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
		The package now is compatible with polyglossia (Joachim Breitner).
		Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

==> preamble.tex <==
\usepackage{xspace}

%Here we define a marco: The \xspace ensures correct spacing, i.e. insert space before next word, but not before period or comma.
\newcommand{\paxos}{\textsc{Paxos}\xspace}

%These packages are needed for the plot in Figure 1. 
\usepackage{tikz}
\usepackage{pgfplots}
\pgfplotsset{compat=newest}



==> tex/Implementation.tex <==
\begin{figure}[h]
  \centering
  \caption{Overview of the speaker recognition system }
  \includegraphics[width=\linewidth]{fig/meth1.png}
  \label{fig:m1}
\end{figure}

The implementation of a speaker recognition system follows two essential phases: the training phase and the testing phase. In the training phase, we have sample voice signals extracted from each user that we need to identify. In the testing phase, we test each incoming voice signal against the pre-stored users' features and try to guess the identity of the user.

Figure~\ref {fig:m1} illustrates the holistic view of such system. We model the problem as a classification problem of classifying a given voice segment to one of the $N$ stored users. We utilize the training phase to extract the most crucial features from each user and keep that feature mapping for future use. Such feature mapping is known as a codebook. 

The derivation of a codebook follows many steps. For clarity, we present each step as a block. As figure 1 depicts, extract the input from the user. These inputs are pre-extracted and stored under two datasets: a training set and a test set. The given training set consists of eleven users pronouncing the word zero, and a second sample from selected eight users is provided as the test set. Therefore, we read audio files from the corresponding directory depending on the phase. Once the audio file is accessible, we move to the feature extraction block from the voice files. The main problem we face in the feature extraction process is the differences in the duration of the voice signals. The situation can be exacerbated at the testing phase, and robust implementation against such variations is paramount. Similar to many voice recognition work in literature, such as~\cite{Muda2010VoiceRA}, we utilize Mel Frequency Cepstral Coefficient (MFCC), for feature extraction. 

Next, we generate codebooks for extracted features using the clustering-based vector quantization method. In particular, we use LBG algorithm~\cite{1094577}. Once we have a codebook for each user, we move to the testing phase. We elaborate on each block in the rest of the subsections.

\begin{figure}[h]
  \centering
  \caption{Block diagram of a typical MFCC processor }
  \includegraphics[width=\linewidth]{fig/m2.png}
  \label{fig:m2}
\end{figure}

\subsection{Feature extraction}

As we discussed in the previous section, we use MFCC for feature extraction. The figure~\ref{fig:m2} portrays the functional blocks of a typical MFCC processor. In an incoming voice signal, the frequency changes over time. In many applications related to voice, processing after the arrival of the complete signal carries no importance. Therefore, in the beginning, we split the signal into overlapping frames, as it is reasonable to assume that for a given short time period, frequencies of a signal have a stationary property. It is empirically proven that such a method can accurately approximate the Fourier representation of the signal. As in any typical setup, we also represent one frame by ($N$) 256 samples and the number of overlapping samples to ($M$) 100.

Next, we apply a window on top of each frame. The usage of a window helps to mitigate any spectral leakage. There is a copious amount of choices for a window, but we select the most used Hamming window for our implementation. The Hamming window is as follows,

\begin{equation}
    w[n] = 0.54 - 0.46cos(2\pi n/(N - 1))
\end{equation}

After applying the window, we take the Fourier Transform of the result. We can use the Fast Fourier Transform (FFT) as it is readily available in many languages or computer programming platforms. We deviate a little from the traditional approaches and compute the power spectral density (PSD) as it provides better and deterministic characteristics than FFT~\cite{fayek2016}. The PSD is calculated using the following equation.  

\begin{equation}
    PSD = \frac{|FFT(frame_i)|^2}{N}
\end{equation}
Where, $frame_i$ is the $i^{th}$ frame of the split signal. 

Next, we exploit the property of human ear sensitivity for our model. In fact, the human ear has a non-linear perception and this can be modeled using filter banks in the Mel domain (figure~\ref{fig:m3}). For this, we use the following map to convert the frequency range of the signal into the Mel frequency domain and extract corresponding filter banks and send PSD frames through filter banks.

\begin{equation}
    m_f = 2595 \log( 1 + \frac{f}{700})
\end{equation}

\begin{figure}[h]
  \centering
  \caption{Mel frequency filter banks }
  \includegraphics[width=\linewidth]{fig/w1.png}
  \label{fig:m3}
\end{figure}

As per the final step, we apply discrete cosine transformation on the extracted filter banks. We omit the first coefficient and extract the rest. Furthermore, it is known that for automatic speech recognition, the most crucial information is embedded in cepstral coefficients 2 to 13. The fine details contained in other coefficients have no ( or less) role in our problem and we can safely discard them. 

Apart from these archetypal blocks, we perform some pre-processing at the input of the signal~\cite{Muda2010VoiceRA} and normalization at the output of the feature extraction block. The holistic view of the overall process is illustrated in figure~\ref{fig:m44}. The `Pre-Emphasis' block at the beginning amplifies the high frequencies of the input signal. Implementation of this block provides a good signal-to-noise ratio, stabilizes the numerical calculations of the Fourier Transform, and balances the frequency spectrum. The implementation of the 'Pre-Emphasis' is as follows,

\begin{equation}
    y(t) = x(t) - \alpha x(t-1)
\end{equation}
where $\alpha$ is a constant and $x(t)$ is the input signal. The traditional choice of $\alpha$ is 0.95. But, in our implementation we use $\alpha = 0.99$.

\begin{figure}[h]
  \centering
  \caption{Overall view of the feature extraction process before feature mapping }
  \includegraphics[width=\linewidth]{fig/f4.png}
  \label{fig:m44}
\end{figure}

Figure~\ref{fig:m44} portrays the overall pipeline of the speaker recognition system. In the training and test phases, we follow the discussed process ( up to coefficient normalization block on figure~\ref{fig:m44} ) for each training and test sample separately. We can then use these coefficients to represent the input signal as represented in figure~\ref{fig:m44}. In the following subsection, we elaborate on the process of the derivation of codebooks and speaker recognition using these features.

\subsection{Feature Matching}

\begin{figure}[h]
  \centering
  \caption{Flow diagram of the LBG algorithm}
  \includegraphics[width=\linewidth]{fig/flow.jpg}
  \label{fig:m454}
\end{figure}

After extracting MFCCs from the input voice sample, we should then design a way to recognize the speaker based on these voice features. In this project, we adopt the VQ technique to address the problem owing to its effectiveness, efficiency and robustness.

VQ is a process of mapping vectors from a large vector space to a finite number of regions in that space. Each region is called a cluster and each cluster can be represented by its centroid, or codeword. This process can be accomplished by the well-know LBG algorithm~\cite{1094577}, which cluster a set of $L$ training vectors into a set of $M$ codebook vectors. The algorithm is formally implemented by the following recursive procedure as presented in figure~\ref{fig:m454}. 

To begin with, the algorithm will initialize a single-vector codebook representing the centroid of all training vectors. Then, it will double the size of the codebook by splitting each current codebook $cb_{n}$ according to the following rule

\begin{equation}
    cb_{n}^{+} = cb_{n} (1 + \epsilon)
\end{equation}
\begin{equation}
    cb_{n}^{-} = cb_{n} (1 - \epsilon)
\end{equation}
where $\epsilon$ is a splitting parameter and be set to 0.01 in this project. Afterward, we will update the centroid of each training vector to create a new set of codebooks. We can see that in each iteration, the size of the codebook will be doubled. The algorithm would repeat this process until the number of codebooks meet our requirement. That is, $M=8$ in this project.

\begin{figure*}[h]
  \centering
  \caption{Visualization of LBG clustering algorithm. Black dots represent the features extracted from the voice sample. Green dots represent the centroids (i.e. codebook)}
  \subfigure[Initialize with 1 codebook]{\includegraphics[width=0.45\columnwidth]{fig/1.jpg}}
  \subfigure[Update centroid]{\includegraphics[width=0.45\columnwidth]{fig/1.jpg}}
  \subfigure[Double the codebook by spliting]{\includegraphics[width=0.45\columnwidth]{fig/2.jpg}}
  \subfigure[Update centroids]{\includegraphics[width=0.45\columnwidth]{fig/2.5.jpg}}
  \subfigure[Double the codebook by spliting]{\includegraphics[width=0.45\columnwidth]{fig/3.jpg}}
  \subfigure[Update centroids]{\includegraphics[width=0.45\columnwidth]{fig/3.5.jpg}}
  \subfigure[Double the codebook by spliting]{\includegraphics[width=0.45\columnwidth]{fig/4.jpg}}
  \subfigure[Update centroids]{\includegraphics[width=0.45\columnwidth]{fig/4.5.jpg}}
  \label{fig:1234}
\end{figure*}

Since the obtained features (i.e. MCFFs) is a high dimension vector, it's very challenging to illustrate the data with the plain figure. Thus, in order to better present the algorithm process, we first reduce the dimension of obtained feature into four. Then, pick up two from these four dimensions as the x-axis and y-axis respectively. Finally, we pick up one user from the testing set as an example.

Figure~\ref{fig:1234} depicts the visualization of the LBG algorithm's executing process, where the 192 black dots represent the features extracted from the voice sample we selected of 192 frames, and green dots represent the centroids (i.e. codebook) from the LBG algorithm. From the subfigure (a) to (h), we can see the evolution of codebook in $1^{th}$, $2^{th}$, $3^{th}$ and $4^{th}$ iterations respectively. We can clearly observe the number of centroids split and evolve from 1 to 8 and then the iteration is terminated.

==> tex/abstract.tex <==
% \textbf{This document serves both as a template and a guideline for your report. You can replace headings and body text with your content. Before you start writing, however, we recommend that you carefully consider the instructions in this document.
% }

% The abstract describes in concise words what you do, why you do it (not
% necessarily in this order), and the main result. The abstract
% has to be self-contained and readable for a person in the
% general area. We suggest to write the abstract first,
% as a means to guide the work, but it should be updated continuously.
% This work is a regeneration of the original work of the paper titled `Optimal Skampling for the Flow Size Distribution', by Darryl Veitch and Paul Tune, which was published on the IEEE Transactions on Information Theory, June 2015. 
Speaker recognition is a popular yet challenging task. In the recent past, an amelioration of work related to audio processing became prolific, especially with the burgeoning popularity of machine learning and deep learning techniques combined with effortless access to large datasets. In this project, we implement a voice recognition system, which is very accurate and efficient, but a simple approach uses no machine learning or deep learning techniques. In fact, we show that our implementation yields 100\% recognition accuracy in both training and test sets. 

==> tex/architecture.tex <==
% In this section, we present a generic model for Flow Sampling and Sketching (FSS). Then, we upgrade the FSS model to Optimal Flow Sampling and Sketching by following the ideas presented in the paper~\cite{veitch2015optimal}.

% \subsection{Flow Sampling and Sketching (FSS)}
% \begin{figure}[h]
%   \centering
%   \caption{Illustration of the FSS pipeline }
%   \includegraphics[width=\linewidth]{fig/flow.pdf}
%   \label{fig:flow}
% \end{figure}

% Figure~\ref{fig:flow}, illustrates the FSS pipeline in a network setup. For each incoming packet, a hash key is calculated using a hash function. The generation of the hash key is done by extracting payload fields such as source port, destination port, source address, destination address, etc. It is ideal to use a hash function that can map each packet with an i.i.d. Once we have the hash value, we can decide whether to sample the given packet or simply drop it. If the packet belongs to a selected flow, we can use the same hash key to locate the corresponding location of that flow in the sketching array. A sketching array is essentially an array initiated with all zeros. The idea behind sketching is to increase the counter value at the corresponding cell, each time you receive a new packet from the same flow. As described in  section~\ref{sec:method}, we have to expect collision as the counter sketch array is of a fixed size. After increasing the counter value, we can safely drop the packet without being an overhead. Once we have the sketch, we can utilize the ideas from (~\cite{Kumar} and ~\cite{veitch2015optimal}) to generate the flow size distribution.

% \subsection{Optimal Flow Sampling and Sketching (OFSS) }
% It is straight forward to update FSS into OFSS. Once we calculate the $p_f^*$ and $\alpha^*$, we can use the same FSS pipeline with $p_f^*$ and $\alpha^*$. 

==> tex/background.tex <==
Give a short, self-contained summary of necessary background
information. 

For our example if your project is a new \paxos implementation, the background
would be a brief introduction to the consensus problem, the \paxos algorithm,
the system model used by the \paxos algorithm
and common optimizations and relevant variations of that algorithm.

The goal of the background section is to make the paper 
self-contained for an audience as large as possible. As in every
section you start with a very brief overview of the section.
For our example that would be: In this section, we introduce the consensus problem,
the \paxos algorithm and common optimizations of that algorithm.

If you copy a definition from a text book or some other source, you must cite that source. 
See Example~\ref{def:consensus} below. 


==> tex/citations.tex <==
It is important that you correctly refer to sources. 

\begin{itemize}
\item If you describe background, according to some textbook, cite that textbook. \emph{See Example~\ref{def:consensus} below.}
\item If you make a claim about trends in industry or research, add citations to validate the claim. \emph{See Example~\ref{ex:trend} below.}
\item \textbf{Do not copy paste text from any source into your report without citation. It will be considered plagiarism.}
\item Always use the tilde character between the text and the cite command, e.g.:\begin{verbatim}
DBLP~\cite{dplg}
\end{verbatim}
The tilde inserts a space, but prevents line break between the text and citation.
\item For correct citations we recommend that you export bibtex entries from DBLP~\cite{dplg}. 
%@Hein: ACM produces crappy doi-urls for non ACM publications. I do believe that there are few papers that are part of the ACM-DL and not in DBLP.
But make sure to update the bibtex entries to adhere to the following rules.
\end{itemize}

Here are some rules to be followed for your bibliography:

\begin{itemize}
\item Make sure titles are correctly capitalized.

%You can export all nsdi citations from DBLP, accordingly this should not be a problem.
% \item Make sure abbreviations are consistent (e.g., is NSDI spelled out or
% not?) - using the @abbrev function in latex helps here.

\item Make sure there is enough info for a reader to find the document: authors
plus title isn't enough.

\item Don't blindly copy and paste ACM bibtex entries without fixing them:

- they list "New York, NY" as the address field, which means that all ACM
conferences look like they took place there; just delete this, or - better

- replace it with where the conference took place, which is much more
helpful to the reader than the publisher's address

- they have a truly weird idea about how to capitalize conference names;
just correct this (consistently)

* IEEE is equally bad, and uses a partially-inverted form of conference
names.

* Please actually review the bibliography before submitting your paper!
\end{itemize}

%@Leander: Move this to the Latex part:

And while you are at it, please:

\begin{itemize}
\item Add include{mathpmtc} in the main LaTeX file, so you don't have
math stuff in a different font than the main text. 
%We could simply add this to the template if not already done.

\item Always use the tilde character between the number and unit, e.g. 100~Mbps or 53~ms. 
The tilde inserts a space, but prevents line break between the number and unit.

\item Never put SI units in italics. 

\item Do differentiate between bits (b) and bytes (B), and between powers of 10~(MB) and 2~(MiB).

\item Avoid things like: "We refer the reader to [42]." That is, don't use citations as nouns.
\end{itemize}


\begin{example}
\label{def:consensus}
Consensus is a distributed programming abstraction that fulfills the following properties~\cite{aTextbook}:
\begin{description}
\item[Termination]
\item[Validity]
\item[Integrity]
\item[Agreement]
\end{description}
\end{example}

\noindent
\begin{example}
\label{ex:trend} Consensus systems build a fundamental part of todays cloud-computing infrastructure~\cite{spanner,chubby,zookeeper,zookeeperWeb}.
\end{example}



==> tex/conclusion.tex <==
In this project, we explored the concurrent use of Digital Signal Processing and pattern recognition in identifying the user of a given voice segment. Among an ample number of methods, we utilize the use of a simple and very efficient approach of vector quantization and show ideal performance in given datasets. We see such a method can achieve expected accuracy with no leverage on computation complexity, memory usage, and execution time. 

==> tex/further.tex <==
Here are some other useful resources: (make these into references instead of links?)
\begin{itemize}
\item The co-chairs of the Ninth SOSP prepared some recommendations and valuable lessons in a paper titled \textit{How (and How Not) to Write a Good Systems Paper} \url{https://www.usenix.org/legacy/publications/library/proceedings/dsl97/good_paper.html}
\item \url{http://gramoli.redbellyblockchain.io/web/doc/talks/researchmethod.pdf}
\item \url{https://www.doc.ic.ac.uk/~prp/doc/talks/11-prp-paper_writing.pdf}
\item This template is inspired by a template from Markus P\"uschel~\cite{puschel}.

\end{itemize}

==> tex/introduction.tex <==

\noindent
% Speaker recognition is the process of identifying the user based on information from a given speech segment. This technique makes it possible to use the speaker's voice to verify their identity for authentication of access. In this final project, we have implemented a speaker recognition system that learns from a set of speakers’ and identifies if there’s a known speaker in a given voice segment. Our speaker  recognition process is realized with digital signal processing method. Specifically, it can be broken down into two main parts: speech feature extraction and speech feature matching. 
Speaker recognition is the process of identifying the user based on extracted information from a given speech sample. This technique makes it possible to use the speaker’s voice to verify their identity for authentication purposes. In this project, we have implemented a speaker recognition system using Digital Signal Processing (DSP) techniques that can learn from a set of speakers and identify if there is a known speaker in a given voice sample. 

Specifically, our system can be broken down into two main parts: speech feature extraction and speech feature matching. We first adopt Mel-frequency Cepstrum Coefficients (MFCCs) ~\cite{Muda2010VoiceRA} to extract a robust representation of a given voice sample (i.e. features). Then, the extracted features are used to generate codewords through the well-known Linde, Buzo, and Gray (LBG) Algorithm ~\cite{1094577}. Finally, based on the concept of Vector Quantization (VQ), we match the MFCCs obtained from a given voice sample with the resulting codebook to classify and identify the corresponding speaker.
%Specifically, we use Digital Signal Processing (DSP) techniques to generate . Then we apply pattern recognition techniques to classify and identify the user. 

The content of this report is organized as follows. Firstly, Section 2 presents the design details and our methodology for the speaker recognition system, including feature extraction and feature matching. Afterward, Section 3 evaluates and shows the performance of our system by conducting experiments on several data sets. Section 4 discusses and provides more insight into our evaluation result. Finally, Section 5 summarizes and closes this work with conclusions.
%The immense advancement of technologies related to network hardware and software has reached a point where high speed (40 Gbps or more) line rates are now available for enterprise-scale networks. While this is good news for the users, traffic monitoring and decision-making have become challenging for the network operators due to the available inefficient sampling methods to handle the sheer volume of data traversing in the network. This contemporary problem has placed a question mark on the capabilities of the existing sampling techniques and other data extracting mechanisms. At the same time, the requirement of an efficient sampling technique is paramount to almost all fields ranging from commercial enterprises to scientific research. Many exciting works in these areas are now available, especially video classification using network traffic~\cite{Biernacki2019}, usage of different machine learning algorithms to understand and classify network traffic~\cite{8748290}, etc. 

%To address such problems, the authors of the paper~\cite{veitch2015optimal} propose a novel methodology encompassing the aspects of both flow sampling and sketching, which is known as skampling to exploit the inherent favorable properties of each sampling and sketching techniques. Therefore, in this project our main focus is to reproduce some of the work presented in the paper~\cite{veitch2015optimal} by implementing their algorithms and evaluating the results by comparing generated figures with the original figures.
% The introduction is different from the abstract; it should elaborate
% more on the context of the work and other aspects. Generally, you can repeat some
% of the main points also in the introduction, but expand and use different words.


% To make your report easier to read, we recommend that you write in first person,
% plural, i.e.~write \textit{we}, even if the report is single author.
% This is also to represent that, even though you are writing this on your own,
% your supervisor and possibly others are contributing ideas, suggestions and
% corrections on your report.

% What follows is a possible structure of the introduction.
% Note that the structure can be modified, but the content should be the same.
% Introduction and Abstract should fill at most the first page.

% \paragraph{Context and Motivation} The first few sentences in the introduction
% is typically a brief description providing context for your work, explaining
% the broader domain of the work. This context should lead into the motivation for
% the work by identifying one or more problems. 

% Here is an example from~\cite{zorfu}:

% \textit{Traditional desktop applications, such as word processing, email, and photo management are increasingly moving to server-based deployments. However, moving applications to the cloud can reduce availability because Internet path availability averages only two-nines~\cite{internetPaths}. If a user's application state is isolated on a single server, the availability for that user is limited by the path availability between the user's desktop and that server. Hence, to improve availability, application state must be replicated across multiple servers placed in geographically distributed data centers.}

% \paragraph{Research Problem} This paragraph further restricts the problem introduced in the motivation to the problem you are addressing. 
% Make sure to explain to the reader 
% what you are doing, why it is important, and why it is non-trivial.

% \paragraph{Related Work} Next, you have to give a brief overview
% of related work. For a paper like this, anywhere between 2
% and 8 references. Briefly explain what they do. End the paragraph by
% contrasting their work to what you do, to make it precisely clear what
% your contribution is.

% \paragraph{Contribution Summary} 
% It can be a good idea to end the introduction with a summary of your contributions as bullet points.
% For example:
% \begin{itemize}
% \item We implement \paxos using brand new technologies.
% \item We evaluate our implementation both in a WAN and LAN environment and show that it is $1.0001\times$ faster than state of the art.
% \end{itemize}
% It is not necessary to have a paragraph at the end of the introduction, that lists the following sections. 


==> tex/latex.tex <==
One of the key features of a speaker recognition system is to make a binary decision to handle inputs from unknown users. Therefore, we plan to include a binary decision at the beginning of the speaker recognition system in the next phase, as it is vital to detect whether the user already exists. The idea is to alleviate the miss classification of an unknown user with the existing users. For such implementation we expect access to more data to create a separate codebook for negative samples ( i.e. unknown users ). The empirical results suggest that thresholding on minimum distance cannot solely handle such decisions, but can detect if the user has a very distinctive accent.

==> tex/method.tex <==
\begin{algorithm}[h]
\caption{Huffman Coding}\label{alg:cap}
\begin{algorithmic}
\Require $ originaltext, D $ \Comment{Default value 2}

%\Ensure $y = x^n$
\State $T \gets originaltext$
\State $D \gets D$
\For {each $char$ in $originaltext$}
    \State $map \gets (char, count)$
\EndFor
\State $sorted\_values \gets sort(map[count])$
\State $probs \gets sorted\_values/sum(sorted\_values)$ \Comment{Element-wise division}
\State $m \gets length(map[keys])$
\State $dummy \gets remainder(m-1,D-1)$
\State $steps \gets (m-1 + dummy)/(D-1)$
\State $CA \gets ones(m+dummy,steps+1).*2$
\State $CA[:,1] \gets probs$
\For{$i = 1 : steps$}
    \State $C \gets CA[:,i]$
    \State $I \gets mins(C,D)$\Comment{D number of indices of minimum values from the last index to index 1}
    \State $SP \gets sum(C[I])$
    \State $MI \gets min(I)$
    \If{$i$ is 1 $ \lor I[k] \not\in mapN$}% {$i = 1$ }\OR $I[k]$ not in $mapN$
        \State $mapN \gets (I[k],MI)$
    \Else
        \For{each $key$ in $mapN$}

            \For{each $j$ in $I$ }
                \If{$j \in mapN[key]$}
                    \State $mapN[key] \gets [mapN[key],MI]$
                \EndIf
            \EndFor
            \EndFor

    \EndIf
    \State $CA[:,i+1] \gets C$
    \State $CA[MI,i+1] \gets SP$
\EndFor
\State $avg\_len \gets 0$
\For{ i = 1 : length(probs)}
    \State $ avg\_len \gets avg\_len + probs[i]*numel(mapN[i])$
\EndFor
\end{algorithmic}
\end{algorithm}
% \While{$N \neq 0$}
% \If{$N$ is even}
%     \State $X \gets X \times X$
%     \State $N \gets \frac{N}{2}$  \Comment{This is a comment}
% \ElsIf{$N$ is odd}
%     \State $y \gets y \times X$
%     \State $N \gets N - 1$
% \EndIf
% \EndWhile
% \end{algorithmic}
% \end{algorithm}
We approach the problem by first creating the alphabet and the corresponding probability of the occurrence of each distinct symbol. This is achieved using the 'map` object in Matlab. We scan the input text and extract each distinct symbol ( letters, white spaces, punctuation, etc.) and their count. Then, we find the relative occurrence of each symbol by dividing each count by the sum of the total count and sorting the probabilities and the symbols respectively. In a more general approach, we might have to use dummy symbols depending on the value of $D$. To handle this, let $m$ be the number of distinct symbols then the number of dummy symbols required is given by,
\begin{equation}
    dummy = (m-1)\bmod(D-1)
\end{equation}
Then number of steps in the process is given by,
\begin{equation}
    steps = (m - 1 + dummy)/(D-1)
\end{equation}
We then initialize a matrix $CA$ with each entry equal to 2 and change the first column with the sorted probabilities calculated in the previous step. Next, we iterate through each step extracting the indices of the minimum $D$ number of probabilities from the (say $i^{th}$ column) $CA$. We maintain a separate map object to track connected nodes ($mapN$), where the key is a string, and the value is an array representing all the nodes that are connected up to this step. After extracting the minimum probabilities, we check whether any of the indices are inside any of the keys and update that key by appending the new minimum index of extracted indices. Also, we initialize a key-value pair if any of these indices are new. Finally, we copy probability values of the $i^{th}$ column to the $(i+1)^{th}$ column, but up to the row index equals to the minimum index we calculated earlier, and we update the data index of the row with the sum of the minimum probabilities we calculated previously. We continue this process, $steps$ number of steps, and we converge to the sum of probabilities equals 1. The proposed algorithm is given in Algorithm~\ref{alg:cap}.



% Now comes the "beef" of the paper, where you explain what
% you did. Again, organize it in paragraphs with titles. As in
% every section you start with a very brief overview of the
% section. 

% This section may vary significantly depending on your topic.
% You may also choose to make the different parts individual sections.
% Here is a more general structure:

% \subsection{Design} Concisely present your design. Focus on novel aspects,
% but avoid implementation details. Use pseudo-code and figures to better
% explain your design, but also present and explain these in the text.
% %
% To assist in evaluating your design choices, it may be relevant to describe
% several distinct \textit{design alternatives} that can later be compared.

% \subsection{Analysis} Argue for the correctness of your design and 
% why you expect it to perform better than previous work.
% %
% If applicable, mention how your design relates to theoretical bounds.

% \subsection{Optimization} Explain how you optimized your design and 
% adjusted it to specific situations.
% %
% Generally, as important as the final results is to show
% that you took a structured, organized approach to the optimization
% and that you explain why you did what you did.
% %
% Be careful to argue, why your optimization does not break the 
% correctness of your design, established above.
% %
% It is often a good strategy to explain a design or protocol in stepwise refinements,
% so as to more easily convince the reader of its correctness. 

% \subsection{Implementation} It is not necessary to "explain" your code. 
% However, in some cases it may be relevant to highlight 
% additional contributions given by your implementation.
% Examples for such contributions are:
% \begin{itemize}
% \item \emph{Abstractions and modules}: If your implementation is nicely separated into interacting
% modules with separated responsibilities you could explain this structure,
% and why it is good/better than some other alternative structure.
% \item \emph{Optimization}: If you spend significant time optimizing your code, e.g.~using profiling tools,
% the result of such optimization may be presented as a contribution. In this case, reason, 
% why the optimized code works better.
% \item \emph{Evaluation framework}: If you implemented a framework or application to evaluate your implementation against existing work, or in a specific scenario, this framework may be presented as a contribution.
% \end{itemize}

% Make sure to cite all external resources used.


==> tex/results.tex <==
In this section, we present the performance of our implementation under several experiments. We have used several datasets for evaluation purposes. The original dataset contains eleven training samples representing eleven users, and the testing set have eight samples from eight selected users as mentioned above. In each sample a single user pronounces the word `` zero ''. We extend the dataset by including our own voices and in some cases with test samples contains pronunciation of other words than zero. 


\subsection{Evaluation on the original training set}

The training accuracy of the model is calculated after extracting codebooks for each user. In the process of training set evaluation, we simply load training samples and calculate their MFCC. The calculated MFCC is then compared with the pre-stored user codebooks and find the distance from each sample to the saved codebooks. 

Table~\ref{tab:tab1} illustrates the distance calculated from each training sample to such user codebooks. We use Euclidean distance as the metric to evaluate the similarity. From table~\ref{tab:tab1}, we see that all the diagonal elements hold the minimum value for each row. This implies that our speaker recognition system can identify all of the speakers in the training samples accurately (i.e. 100\% training accuracy). 

\subsection{Evaluation on the original testing set}

After having desired performance on the training set, we evaluate our model on the testing set. The provided testing set is imbalance and has only eight data points representing the first eight users. 

Table~\ref{tab:tab2} summarizes the overall performance of the model against the testing set. We see similar behavior to the training set evaluation and our speaker recognition system correctly identifies all the testing users (i.e. 100\% testing accuracy). This result preliminarily verifies the effectiveness of our speaker recognition system.

\begin{table*}[ht]
  \resizebox{\textwidth}{!}{\begin{tabular}{*{13}{c}}
    \toprule
  True user & s1 & s2 & s3 & s4 & s5 & s6 & s7 & s8 & s9 & s10 & s11 & Prediction\\
    
    % &  &\multirow{3}{*}{MSA}  & \multirow{3}{*}{MSA} & \multirow{3}{*}{MSA} \\
    % & &  & & & \\
    % & &(\%) & (\%) &  (\%)\\
    \midrule
    s1 & \textbf{0.0726} &   0.0876  &  0.0960  &  0.0841 &   0.0837 &   0.0873  &  0.0818  &  0.0848  &  0.0886 &   0.1136  &  0.1198 &  s1\\
    s2 & 0.0824 &   \textbf{0.0666} &   0.0867  &  0.0810  &  0.0945  &  0.0989  &  0.0910  &  0.0974 &   0.1014 &   0.0972  &  0.1028  & s2 \\
    s3 & 0.0917 &   0.0875 &   \textbf{0.0635}  &  0.0873  &  0.1022  &  0.0897   & 0.0859 &   0.0964 &   0.1017 &   0.0959  &  0.0982 & s3 \\
    s4 & 0.0826  &  0.0837 &   0.0933  &  \textbf{0.0705} &   0.0917 &   0.0949  &  0.0847  &  0.0852 &   0.0960  &  0.1032&    0.1143 &  s4\\
    s5 & 0.0779 &   0.0959  &  0.1022 &  0.0898  &  \textbf{0.0664}  &  0.0862  &  0.0878  &  0.0816  &  0.0808  &  0.1136 &   0.1179 & s5\\
    s6 & 0.0848  &  0.1032  &  0.0952  &  0.0925 &   0.0865   & \textbf{0.0729} &   0.0799  &  0.0801  &  0.0846  &  0.1095  &  0.1108 & s6\\
    s7 & 0.0816  &  0.0995 &   0.0950 &   0.0855  &  0.0921   & 0.0825  &  \textbf{0.0690}  &  0.0797  &  0.0875  &  0.1094 &   0.1180 & s7 \\
   s8 &  0.0834 &   0.1029  &  0.1002  &  0.0863  &  0.0841 &   0.0839  &  0.0794  &  \textbf{0.0719} &   0.0840 &   0.1101  &  0.1138 & s8\\
    s9 & 0.0893  &  0.0985  &  0.1074  &  0.0965 &   0.0829  &  0.0951 &   0.0892  & 0.0845  &  \textbf{0.0709} &   0.0939 &   0.0918 & s9\\
     s10 &  0.0982  &  0.0922  &  0.1013 &  0.0969  &  0.0870 &   0.1093  &  0.0951  &  0.0939  &  0.0853 &   \textbf{0.0664}  &  0.0743 & s10\\
      s11 &  0.0991  &  0.0911  &  0.0923  &  0.0968  &  0.0925 &    0.1074  &  0.0994  &  0.0968   & 0.0894  &  0.0738 &   \textbf{0.0613} & s11\\
    
  \bottomrule
\end{tabular}}
\caption{Performance of the speaker recognition system against the training set. Each row illustrates the distance from the training sample to each training user. If we concentrate on the diagonal elements we get the minimum distance for that row. The column corresponding to the minimum distance in each row is re-coded as the predicted user. Here the distance is the $L_2$ norm. }
 \label{tab:tab1}
\end{table*}


\begin{table*}[ht]
  \resizebox{\textwidth}{!}{\begin{tabular}{*{13}{c}}
    \toprule
  True user & s1 & s2 & s3 & s4 & s5 & s6 & s7 & s8 & s9 & s10 & s11 & Prediction\\
    
    % &  &\multirow{3}{*}{MSA}  & \multirow{3}{*}{MSA} & \multirow{3}{*}{MSA} \\
    % & &  & & & \\
    % & &(\%) & (\%) &  (\%)\\
    \midrule
    s1 & \textbf{0.0737} &   0.0901 &    0.1020  &   0.0831 &    0.0789  &   0.0881  &   0.0799   &  0.0800  &   0.0881  &   0.1145 &    0.1215 &  s1\\
    s2 & 0.0837 &   \textbf{0.0726}  &  0.0858  &  0.0812  &  0.0949 &   0.0976  &  0.0893  &  0.0951  &  0.0993  &  0.0966 &   0.1040  & s2 \\
    s3 & 0.0893  &  0.0885  &  \textbf{0.0799}  &  0.0883 &   0.0929  &  0.0953  &  0.0859  &  0.0913  &  0.0913  &  0.0956 &   0.1019 & s3 \\
    s4 & 0.0813  &  0.0880  &  0.0903  &  \textbf{0.0795}  &  0.0891  &  0.0924  &  0.0825  &  0.0839  &  0.0931   & 0.1064 &   0.1134 &  s4\\
    s5 & 0.0800  &  0.0951  &  0.0943  &  0.0880  &   \textbf{0.0754}  &  0.0814  &  0.0854  &  0.0836  &  0.0845  &  0.1139  &  0.1183 & s5\\
    s6 & 0.0810  &  0.0993  &  0.0912 &   0.0920 &   0.0882  &  \textbf{0.0708}  &  0.0789  &  0.0817 &   0.0884  &  0.1152 &   0.1133 & s6\\
    s7 & 0.0816  &  0.0955 &   0.0942   & 0.0838  &  0.0872 &    0.0864  &  \textbf{0.0742}  &  0.0788  &  0.0876   &  0.1115 &   0.1191 & s7 \\
   s8 &  0.0852  &  0.1010  &  0.0976  &  0.0868   & 0.0826  &  0.0807  &  0.0816 &   \textbf{0.0752} &   0.0853  &  0.1103  &  0.1137 & s8\\
    
  \bottomrule
\end{tabular}}
\caption{Performance of the speaker recognition system against the test set. Each row illustrates the distance from the testing sample to each trained user. If we concentrate on the diagonal elements we get the minimum distance for that row. The column corresponding to the minimum distance in each row is recoded as the predicted user. For example, if the true user is s4 (row), the minimum distance calculated across all the users is 0.0795 and it corresponds to the user s4 (column). Here the distance is the $L_2$ norm.}
 \label{tab:tab2}
\end{table*}

% \subsection{Evaluation on an extended test set}
% We extend the test and training sets by adding our own voices as new users. The overall results are illustrated in the table~\ref{tab:tab41}. We see that our speaker recognition system performs very accurately and identify all the 10 test users accurately. Hence, the testing accuracy remains at 100\%.

\subsection{Evaluation on introducing new users}
In this subsection, we further analyze the effect of introducing new users to our speaker recognition system by adding voice samples from two group members to the original training and testing set. Specifically, s12 and s13 are voice samples from Achintha and Chih-ho respectively. 

The evaluation result is illustrated in Table~\ref{tab:tab3}. We can see that our system successfully recognizes all of the users in the testing set. However, since the number of new users is limited in our experiment, we can only conclude that the performance of our system can preserve robustness to new users when the number of total users in the data set remains low. Hence, the testing accuracy remains at 100\%.


\begin{table*}[ht]
  \resizebox{\textwidth}{!}{\begin{tabular}{*{15}{c}}
  
    \toprule
   User & s1 & s2 & s3 & s4 & s5 & s6 & s7 & s8 & s9 & s10 & s11 & s12 & s13 & Prediction\\
    
    \midrule
    s1 &\textbf{0.0599} & 0.0732 & 0.0829 & 0.0676 & 0.0642 & 0.0716 & 0.0650 & 0.0651 & 0.0716 & 0.0931 & 0.0988 & 0.0956 & 0.0913 & s1 \\
    s2 & 0.0685&\textbf{0.0594}&0.0702&0.0664&0.0776&0.0799&0.0730&0.0778&0.0812&0.0790&0.0851&0.0982&0.0836  & s2 \\
    s3 &  0.0740&0.0733&\textbf{0.0662}&0.0732&0.0770&0.0790&0.0712&0.0757&0.0757&0.0793&0.0845&0.0903&0.0807 & s3 \\
    s4 & 0.0663&0.0718&0.0737&\textbf{0.0649}&0.0726&0.0754&0.0673&0.0684&0.0759&0.0868&0.0925&0.0930&0.0914 &  s4\\
    s5 & 0.0651&0.0774&0.0767&0.0716&\textbf{0.0614}&0.0663&0.0695&0.0680&0.0687&0.0927&0.0963&0.0995&0.0869 & s5\\
    s6 & 0.0659&0.0807&0.0741&0.0748&0.0717&\textbf{0.0576}&0.0642&0.0664&0.0719&0.0937&0.0921&0.0865&0.1004 & s6\\
    s7 & 0.0664&0.0777&0.0766&0.0682&0.0709&0.0703&\textbf{0.0604}&0.0641&0.0713&0.0907&0.0969&0.0997&0.0869 & s7 \\
    s8 & 0.0698&0.0827&0.0800&0.0711&0.0677&0.0661&0.0668&\textbf{0.0616}&0.0699&0.0904&0.0931&0.0935&0.0873 & s8\\
    s12 & 0.0750&0.0746&0.0818&0.0805&0.0733&0.0820&0.0731&0.0725&0.0738&0.0775&0.0756&\textbf{0.0658}&0.0946 & s12\\
    s13 & 0.0826&0.0808&0.0839&0.0780&0.0766&0.0889&0.0796&0.0796&0.0688&0.0700&0.0766&0.0902&\textbf{0.0442} & s13\\
  \bottomrule
\end{tabular}}
\caption{Performance of the speaker recognition system against the new test set. We introduce new two voices to both the training set and the test set (Our own voices). These new users are named as \textbf{s12} and \textbf{s13}. We see our system perform 100\% in this scenario as well. }
 \label{tab:tab3}
\end{table*}

\begin{table*}[h]
  \resizebox{\textwidth}{!}{\begin{tabular}{*{15}{c}}
  
    \toprule
   User & s1 & s2 & s3 & s4 & s5 & s6 & s7 & s8 & s9 & s10 & s11 & s12 & s13 & Prediction\\
    
    \midrule
    s1 &\textbf{0.0535}&0.0779&0.0906&0.0655&\textcolor{blue}{0.0536}&0.0736&0.0594&0.0645&0.0660&0.0941&0.1091&0.0986&0.0936 & s1 \\
    s2 & 0.0669&\textbf{0.0528}&0.0661&0.0610&0.0738&0.0847&0.0723&0.0807&0.0834&0.0810&0.0901&0.0995&0.0877  & s2 \\
    s3 &  0.0802&0.0767&\textbf{0.0619}&0.0687&0.0735&0.0872&0.0722&0.0791&0.0762&0.0738&0.0876&0.0901&0.0729 & s3 \\
    s4 & 0.0629&0.0712&0.0774&\textbf{0.0584}&0.0620&0.0797&0.0602&0.0683&0.0721&0.0894&0.1063&0.0984&0.0937 &  s4\\
    s5 & 0.0626&0.0866&0.0792&0.0629&0.0576&0.0649&\textbf{0.0540}&0.0614&0.0637&0.0979&0.1169&0.1070&0.0853 & \textcolor{red}{s7}\\
    s6 & 0.0627&0.0851&0.0774&0.0732&0.0651&\textbf{0.0540}&0.0573&0.0642&0.0651&0.0998&0.1036&0.0855&0.1072 & s6\\
    s7 & 0.0668&0.0822&0.0844&0.0616&0.0574&0.0736&\textbf{0.0560}&0.0629&0.0652&0.0918&0.1129&0.1084&0.0769 & s7 \\
    s8 & 0.0708&0.0916&0.0868&0.0704&0.0615&0.0659&0.0583&\textbf{0.0600}&\textcolor{blue}{0.0603}&0.0926&0.1070&0.0954&0.0795 & s8\\
    s12 & 0.0757&0.0707&0.0943&0.0754&0.0706&0.0943&0.0700&0.0717&0.0666&0.0750&0.0726&\textbf{0.0484}&0.1148 & s12\\
    s13 & 0.0847&0.0883&0.0622&0.0672&0.0705&0.0813&0.0686&0.0760&0.0745&0.0803&0.1051&0.1129&\textbf{0.0283} & s13\\
  \bottomrule
\end{tabular}}
\caption{Performance of the speaker recognition system when we use different phrases in the testing data of s13, where the data points in blue represent the distance that is very close to the groud-truth value. Predictions that are labeled in red imply false prediction.}
 \label{tab:tab4}
\end{table*}

\begin{table*}[h]
  \resizebox{\textwidth}{!}{\begin{tabular}{*{13}{c}}
    \toprule
  True user & s1 & s2 & s3 & s4 & s5 & s6 & s7 & s8 & s9 & s10 & s11 & Prediction\\
    
    % &  &\multirow{3}{*}{MSA}  & \multirow{3}{*}{MSA} & \multirow{3}{*}{MSA} \\
    % & &  & & & \\
    % & &(\%) & (\%) &  (\%)\\
    \midrule
    s1 & 0.0795  &  0.0857 &   0.1004 &   \textcolor{blue}{0.0767}  &  0.0799  &  0.0948 &   0.0834  &  0.0812  &  0.0932 &   0.1099 &   0.1154 &  \textcolor{red}{s4}\\
    s2 & 0.0812  &  \textbf{0.0756}  &  0.0827  &  0.0814  &  0.0885 &   0.0943  &  0.0862 &   0.0899 &   0.1036  &  0.1032  &  0.1133  & s2 \\
    s3 &  0.0846  &  0.0873 &   \textbf{0.0782} &  0.0859  &  0.0870 &   0.0911  &  0.0818  &  0.0852 &   0.1022   & 0.1052  &  0.1116 & s3 \\
    s4 & 0.0818  &  0.0873  &  0.0889 &   \textbf{0.0775}   & 0.0863  &  0.0937  &  0.0834  &  0.0802 &   0.1000 &   0.1075  &  0.1133 &  s4\\
    s5 & 0.0822   & 0.0901 &   0.0935  &  0.0833  &  \textbf{0.0783} &    0.0884  &  0.0873  &  0.0852  &  0.0897 &   0.1080 &   0.1140 & s5\\
    s6 & 0.0785  &  0.0936  &  0.0835  &  0.0877 &   0.0858  &  \textbf{0.0707}  &  0.0756  &  0.0775 &   0.1046  &  0.1212 &   0.1212 & s6\\
    s7 & 0.0832  &  0.0903  &  0.0919  &  0.0800  &  0.0841   & 0.0901  &  \textbf{0.0776}  &  0.0790  &  0.0952 &   0.1113 &   0.1175 & s7 \\
   s8 &  0.0870  &  0.0971  &  0.0940 &   0.0828  &  0.0851   & 0.0855  &  0.0831  &  \textbf{0.0771} &   0.0931  &  0.1070  &  0.1082 & s8\\
    
  \bottomrule
\end{tabular}}
\caption{Performance of the speaker recognition system against the test set without the ` Pre-Emphasis' block. We see a miss classification of the user s1 as user s4. }
 \label{tab:tab5}
 
\end{table*}

\subsection{Evaluation on the effect of different phrases}
Next, we turn to test the ability of our speaker recognition when voice samples that contain different phrase are used. In this experiment, without changing other settings, we replace the test data of s13 with the voice from the same speaker saying a different phrase. 

Table~\ref{tab:tab4} shows the result when s13 speaks "Yes" instead of "zero" in testing data. We can see that the speaker s13 can still be successfully recognized with a distance value of 0.0283 even if the training data and testing data contain a different phrase. However, the recognition ability of other speakers has been affected accordingly. In this case, user s5 is falsely recognized as user s7 while user s1 and user s8 are on the edge of being falsely recognized as user s5 and user s9 respectively. 

We have also tried saying different languages in the voice sample and observed similar results. Specifically, the distance in the table~\ref{tab:tab4} (s13, s13) will become \textbf{0.0289} and \textbf{0.0362} for saying "\textit{Go me na sai}" (i.e. sorry in Japanese) and "\textit{wèi shén me}" (i.e. why in Mandarin) respectively. Thus, we conclude that the recognition can be valid for samples with different phrases when sufficient features can be extracted from the sample.

\subsection{Ablation study}

In this subsection, we perform an ablation study to show the importance of the `` pre-emphasis '' block. As we can see from the table~\ref{tab:tab5}, the model miss classifies user 1 as user 4. Furthermore, if we move along the elements in the rows s6 and s7 in table~\ref{tab:tab5} and compare with the corresponding entries in table~\ref{tab:tab2}, the distance gaps in the entries of table~\ref{tab:tab5} are small. That is, we can strengthen the gaps (i.e. confident levels of the predictions) using the pre-emphasis block.


\subsection{Evaluation on the filtered test data}

In this experiment, we derive a new testing set using the original testing set (i.e. eight users case) and evaluate the robustness of our system against the frequency suppression in testing data. In particular, we use a notch filter centered at the frequency 1000 Hz, and vary the width of the notch filter and evaluate the performance. We first select a value for the width ( as presented in the table~\ref{tab:tab6} ) and create a notch filter and apply it on the testing data to create a new testing set to evaluate the performance. As it is evident from the table~\ref{tab:tab6}, our system stays robust up to approximately a width of 1250 Hz.

\begin{table}[h]
 {\begin{tabular}{*{2}{c}}
    \toprule
  Notch filter width ($f_s/2$ x)& Identified users ( 8 )\\
    
    % &  &\multirow{3}{*}{MSA}  & \multirow{3}{*}{MSA} & \multirow{3}{*}{MSA} \\
    % & &  & & & \\
    % & &(\%) & (\%) &  (\%)\\
    \midrule
    0.1 & 8 \\
    0.2 & 8 \\
    0.3 & 5 \\
    0.4 & 4\\
    0.5 & 4\\
    
    
  \bottomrule
\end{tabular}}
\caption{Performance of the speaker recognition system against filtered test data. Here we have used a notch filter to filer only test data. We vary the width of the notch filter width (factor x $f_s/2$) and applied it at 1000 Hz.}
 \label{tab:tab6}
\end{table}
